Improving Term Evaluation in Machine Translation: Variation Matters

Terminology evaluation in machine translation (MT) usually assumes a single correct target form per source term. However, human translators routinely introduce variation that current metrics penalize as inconsistency. We examine how to account for this variation in document-level MT evaluation of English-French scientific translation, combining glossary-based accuracy, translation consistency, and a new cross-term variation (CTV) diagnostic measure that tests whether variation relationships are preserved across languages. Based on analyses of two parallel corpora, translated by four MT systems, we find that (1) MT systems generate less target-side variation than human translators; (2) transfer patterns strongly depend on the variation type; (3) consistency rankings vary with the choice of metric; and (4) constraining MT with a glossary improves accuracy and consistency but degrades CTV by suppressing valid variation. We argue for variation-aware evaluation that conditions consistency penalties on whether target-side variation mirrors source-side variation.

==> tables/evaluation_coverage/acl/coverage_variation.tex <==
\begin{table*}
\centering
\caption{\%~evaluated by variation category, averaged over documents (\textit{occ}/\textit{dist}; GC = restricted EM)}
\label{tab:coverage_by_cat_doc_avg}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l rr r r r r r r r r}
\toprule
& $\bar{N}_{\text{occ}}$ & $\bar{N}_{\text{dist}}$ & \multicolumn{2}{c}{GC} & \multicolumn{2}{c}{TLC non-EM} & \multicolumn{2}{c}{TLC-EM} & \multicolumn{2}{c}{ITC-var} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Category & & & occ & dist & occ & dist & occ & dist & occ & dist \\
\midrule
no\_variation & 197.9 & 40.2 & 100.0\% & 99.9\% & 90.2\% & 56.6\% & 90.2\% & 56.6\% & --- & --- \\
VR & 24.6 & 6.3 & 43.0\% & 32.2\% & 89.0\% & 66.6\% & 41.7\% & 28.3\% & 31.9\% & 36.6\% \\
VMS & 2.5 & 2.4 & 8.0\% & 7.2\% & 2.3\% & 1.5\% & 2.3\% & 1.5\% & --- & --- \\
VE & 4.1 & 2.2 & 25.7\% & 25.8\% & 31.7\% & 24.4\% & 12.6\% & 11.2\% & 39.5\% & 39.9\% \\
VG & 21.2 & 6.2 & 58.6\% & 47.5\% & 68.7\% & 50.6\% & 52.7\% & 36.0\% & 32.3\% & 34.1\% \\
VL & 21.9 & 10.3 & 35.3\% & 33.1\% & 63.3\% & 38.4\% & 23.5\% & 13.6\% & 31.9\% & 32.2\% \\
CM & 4.8 & 3.1 & 5.3\% & 3.6\% & 25.7\% & 17.1\% & 4.9\% & 3.2\% & --- & --- \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/evaluation_coverage/acl/dimesion_cross_coverage.tex <==
\begin{table*}
\centering
\caption{Cross-method term coverage: average per-document percentage of terms evaluated by $\geq$1 method in each combination. \textit{Cov.} = covered; \textit{Not cov.} = never evaluated by any method in the combination.}
\label{tab:cross_method_coverage}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l rr rr}
\toprule
Method combination & \multicolumn{2}{c}{Covered (\%)} & \multicolumn{2}{c}{Not covered (\%)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& occ & dist & occ & dist \\
\midrule
GC & 85.0\% & 71.7\% & 15.0\% & 28.3\% \\
TLC$_{\neq\text{EM}}$ & 86.9\% & 50.5\% & 13.1\% & 49.5\% \\
TLC$_{\text{EM}}$ & 76.7\% & 41.1\% & 23.3\% & 58.9\% \\
ITC & 9.4\% & 12.5\% & 90.6\% & 87.5\% \\
\midrule
GC + ITC & 91.9\% & 82.6\% & 8.1\% & 17.4\% \\
GC + TLC$_{\neq\text{EM}}$ & 95.1\% & 81.1\% & 4.9\% & 18.9\% \\
GC + TLC$_{\text{EM}}$ & 85.0\% & 71.7\% & 15.0\% & 28.3\% \\
TLC$_{\neq\text{EM}}$ + ITC & 88.7\% & 57.7\% & 11.3\% & 42.3\% \\
TLC$_{\text{EM}}$ + ITC & 83.8\% & 52.5\% & 16.2\% & 47.5\% \\
TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ & 86.9\% & 50.5\% & 13.1\% & 49.5\% \\
\midrule
GC + TLC$_{\neq\text{EM}}$ + ITC & 96.8\% & 87.9\% & 3.2\% & 12.1\% \\
GC + TLC$_{\text{EM}}$ + ITC & 91.9\% & 82.6\% & 8.1\% & 17.4\% \\
GC + TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ & 95.1\% & 81.1\% & 4.9\% & 18.9\% \\
TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ + ITC & 88.7\% & 57.7\% & 11.3\% & 42.3\% \\
\midrule
GC + TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ + ITC & 96.8\% & 87.9\% & 3.2\% & 12.1\% \\
\midrule
\multicolumn{5}{l}{\footnotesize Averaged over 31\,documents. occ = occurrences; dist = distinct terms.} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/evaluation_coverage/acl/evaluated_regarding_dimension.tex <==
\begin{table*}
\centering
\caption{Term coverage overview, averaged per document (\textit{occ} = occurrences, \textit{dist} = distinct terms)}
\label{tab:coverage_overview}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrrl}
\toprule
Metric & \multicolumn{3}{c}{Occurrences (avg/doc)} & \multicolumn{3}{c}{Distinct terms (avg/doc)} & Excl.\ reason \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& $\bar{N}$ & $\bar{N}_{eval}$ & \% & $\bar{N}$ & $\bar{N}_{eval}$ & \% & \\
\midrule
GC-EM$_{restr}$ & 273.9 & 231.3 & 85.0\% & 68.7 & 48.8 & 71.7\% & Source term not found in glossary \\
GC-EM$_{unr}$ & 273.9 & 273.9 & 100.0\% & 68.7 & 68.7 & 100.0\% & N/A \\
\midrule
TLC non-EM & 273.9 & 239.7 & 86.9\% & 68.7 & 34.5 & 50.5\% & hapax (\$k\{=\}1\$): 34.2t/doc \\
TLC-EM & 273.9 & 210.2 & 76.7\% & 68.7 & 27.7 & 41.1\% & hapax (\$k\{=\}1\$): 34.2t/doc; not in gloss.: 6.7t/doc \\
\midrule
ITC-var & 273.9 & 26.7 & 9.8\% & 68.7 & 8.9 & 13.0\% & non-var.: 202.9t/doc; no no\textsubscript\{var\}: 44.3t/doc \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/evaluation_coverage/both_corpora/evaluated_regarding_dimension.tex <==
\begin{table*}
\centering
\caption{Term coverage overview per evaluation dimension, averaged per document (\textit{occ} = occurrences, \textit{dist} = distinct terms).}
\label{tab:coverage_overview}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l rrr rrr | rrr rrr}
\toprule
& \multicolumn{6}{c|}{\ACL} & \multicolumn{6}{c}{\iwslt} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}
& \multicolumn{3}{c}{Occurrences} & \multicolumn{3}{c|}{Distinct terms} & \multicolumn{3}{c}{Occurrences} & \multicolumn{3}{c}{Distinct terms} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
Metric & $\bar{N}$ & $\bar{N}_{eval}$ & \% & $\bar{N}$ & $\bar{N}_{eval}$ & \% & $\bar{N}$ & $\bar{N}_{eval}$ & \% & $\bar{N}$ & $\bar{N}_{eval}$ & \% \\
\midrule
GC-EM$_{restr}$ & 273.9 & 231.3 & 85.0 & 68.7 & 48.8 & 71.7 & 120.3 & 109.2 & 90.4 & 35.2 & 29.3 & 83.3 \\
\midrule
\ITC non-EM & 273.9 & 239.7 & 86.9 & 68.7 & 34.5 & 50.5 & 120.3 & 103.8 & 85.6 & 35.2 & 18.7 & 53.2 \\
\ITC-EM & 273.9 & 210.2 & 76.7 & 68.7 & 27.7 & 41.1 & 120.3 & 96.4 & 79.1 & 35.2 & 16.5 & 46.5 \\
\midrule
\CTV & 273.9 & 26.7 & 9.8 & 68.7 & 8.9 & 13.0 & 120.3 & 3.0 & 2.5 & 35.2 & 1.5 & 4.3 \\

\bottomrule
\end{tabular}
\end{table*}


==> tables/evaluation_coverage/iwslt/coverage_variation.tex <==
\begin{table*}[H]
\centering
\caption{\%~evaluated by variation category, averaged over documents (\textit{occ}/\textit{dist}; GC = restricted EM)}
\label{tab:coverage_by_cat_doc_avg_iwslt}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l rr r r r r r r r r}
\toprule
& $\bar{N}_{\text{occ}}$ & $\bar{N}_{\text{dist}}$ & \multicolumn{2}{c}{GC} & \multicolumn{2}{c}{TLC non-EM} & \multicolumn{2}{c}{TLC-EM} & \multicolumn{2}{c}{ITC-var} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
Category & & & occ & dist & occ & dist & occ & dist & occ & dist \\
\midrule
no\_variation & 88.4 & 24.1 & 100.0\% & 100.0\% & 87.2\% & 54.4\% & 87.2\% & 54.4\% & --- & --- \\
VR & 9.7 & 3.5 & 50.3\% & 45.7\% & 85.0\% & 71.3\% & 46.5\% & 37.2\% & 17.0\% & 20.7\% \\
VMS & 1.0 & 1.0 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & --- & --- \\
VE & 3.5 & 1.5 & 41.7\% & 25.0\% & 41.7\% & 25.0\% & 41.7\% & 25.0\% & 58.3\% & 75.0\% \\
VG & 11.4 & 2.2 & 97.0\% & 90.8\% & 82.4\% & 64.2\% & 82.4\% & 64.2\% & 7.1\% & 11.7\% \\
VL & 7.7 & 3.7 & 40.8\% & 38.7\% & 45.5\% & 31.2\% & 22.2\% & 13.0\% & 8.4\% & 6.6\% \\
CM & 3.7 & 2.0 & 0.0\% & 0.0\% & 27.8\% & 25.0\% & 0.0\% & 0.0\% & --- & --- \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/evaluation_coverage/iwslt/dimesion_cross_coverage.tex <==
\begin{table*}[H]
\centering
\caption{Cross-method term coverage: average per-document percentage of terms evaluated by $\geq$1 method in each combination. \textit{Cov.} = covered; \textit{Not cov.} = never evaluated by any method in the combination.}
\label{tab:cross_method_coverage_iwslt}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l rr rr}
\toprule
Method combination & \multicolumn{2}{c}{Covered (\%)} & \multicolumn{2}{c}{Not covered (\%)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& occ & dist & occ & dist \\
\midrule
GC & 90.4\% & 83.3\% & 9.6\% & 16.7\% \\
TLC$_{\neq\text{EM}}$ & 85.6\% & 53.2\% & 14.4\% & 46.8\% \\
TLC$_{\text{EM}}$ & 79.1\% & 46.5\% & 20.9\% & 53.5\% \\
ITC & 2.7\% & 4.2\% & 97.3\% & 95.8\% \\
\midrule
GC + TLC$_{\neq\text{EM}}$ & 96.9\% & 90.0\% & 3.1\% & 10.0\% \\
GC + ITC & 92.8\% & 87.2\% & 7.2\% & 12.8\% \\
GC + TLC$_{\text{EM}}$ & 90.4\% & 83.3\% & 9.6\% & 16.7\% \\
TLC$_{\neq\text{EM}}$ + ITC & 86.2\% & 55.0\% & 13.8\% & 45.0\% \\
TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ & 85.6\% & 53.2\% & 14.4\% & 46.8\% \\
TLC$_{\text{EM}}$ + ITC & 81.5\% & 50.3\% & 18.5\% & 49.7\% \\
\midrule
GC + TLC$_{\neq\text{EM}}$ + ITC & 97.5\% & 91.9\% & 2.5\% & 8.1\% \\
GC + TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ & 96.9\% & 90.0\% & 3.1\% & 10.0\% \\
GC + TLC$_{\text{EM}}$ + ITC & 92.8\% & 87.2\% & 7.2\% & 12.8\% \\
TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ + ITC & 86.2\% & 55.0\% & 13.8\% & 45.0\% \\
\midrule
GC + TLC$_{\neq\text{EM}}$ + TLC$_{\text{EM}}$ + ITC & 97.5\% & 91.9\% & 2.5\% & 8.1\% \\
\midrule
\multicolumn{5}{l}{\footnotesize Averaged over 10\,documents. occ = occurrences; dist = distinct terms.} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/evaluation_coverage/iwslt/evaluated_regarding_dimension.tex <==
\begin{table*}
\centering
\caption{Term coverage overview, averaged per document (\textit{occ} = occurrences, \textit{dist} = distinct terms)}
\label{tab:coverage_overview_iwslt}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrrl}
\toprule
Metric & \multicolumn{3}{c}{Occurrences (avg/doc)} & \multicolumn{3}{c}{Distinct terms (avg/doc)} & Excl.\ reason \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& $\bar{N}$ & $\bar{N}_{eval}$ & \% & $\bar{N}$ & $\bar{N}_{eval}$ & \% & \\
\midrule
GC-EM$_{restr}$ & 120.3 & 109.2 & 90.4\% & 35.2 & 29.3 & 83.3\% & Source term not found in glossary \\
GC-EM$_{unr}$ & 120.3 & 120.3 & 100.0\% & 35.2 & 35.2 & 100.0\% & N/A \\
\midrule
TLC non-EM & 120.3 & 103.8 & 85.6\% & 35.2 & 18.7 & 53.2\% & hapax (\$k\{=\}1\$): 16.5t/doc \\
TLC-EM & 120.3 & 96.4 & 79.1\% & 35.2 & 16.5 & 46.5\% & hapax (\$k\{=\}1\$): 16.5t/doc; not in gloss.: 2.2t/doc \\
\midrule
ITC-var & 120.3 & 3.0 & 2.5\% & 35.2 & 1.5 & 4.3\% & non-var.: 91.0t/doc; no no\textsubscript\{var\}: 26.3t/doc \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/global_evaluation/global_evaluation_detail/ACL_cometkiwi_type_0.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Document} & EuroLLM-22B-greedy & EuroLLM-9B-greedy & Llama-3.1-8B-greedy & Qwen3-8B-top-p & ref \\
    \midrule
        ACL\_22 & \textbf{0.8650} & 0.8637 & 0.8611 & 0.8626 & 0.8538 \\
        ACL\_21 & 0.8623 & \textbf{0.8642} & 0.8590 & 0.8603 & 0.8408 \\
        ACL\_29 & 0.8676 & \textbf{0.8683} & 0.8623 & 0.8593 & 0.8408 \\
        ACL\_18 & 0.8679 & \textbf{0.8712} & 0.8667 & 0.8663 & 0.8346 \\
        ACL\_5 & 0.8441 & \textbf{0.8466} & 0.8431 & 0.8396 & 0.8326 \\
        ACL\_1 & 0.8444 & \textbf{0.8493} & 0.8467 & 0.8434 & 0.8321 \\
        ACL\_25 & 0.8518 & \textbf{0.8548} & 0.8526 & 0.8492 & 0.8266 \\
        ACL\_9$^{\dagger}$ & \textbf{0.8381} & 0.8346 & 0.8365 & 0.8292 & 0.8250 \\
        ACL\_0$^{\dagger}$ & 0.8363 & \textbf{0.8390} & 0.8308 & 0.8319 & 0.8231 \\
        ACL\_11 & \textbf{0.8498} & 0.8490 & 0.8387 & 0.8437 & 0.8180 \\
        ACL\_7 & 0.8433 & 0.8398 & 0.8343 & \textbf{0.8469} & 0.8143 \\
        ACL\_33 & 0.8474 & \textbf{0.8543} & 0.8450 & 0.8335 & 0.8135 \\
        ACL\_26 & \textbf{0.8524} & 0.8508 & 0.8454 & 0.8493 & 0.8121 \\
        ACL\_14 & \textbf{0.8508} & 0.8467 & 0.8395 & 0.8468 & 0.8087 \\
        ACL\_30 & \textbf{0.8608} & 0.8588 & 0.8552 & 0.8562 & 0.8074 \\
        ACL\_24$^{\dagger}$ & 0.8336 & \textbf{0.8358} & 0.8217 & 0.8291 & 0.8009 \\
        ACL\_27 & \textbf{0.8537} & 0.8413 & 0.8266 & 0.8440 & 0.7988 \\
        ACL\_20$^{\dagger}$ & 0.8263 & \textbf{0.8278} & 0.8163 & 0.8271 & 0.7980 \\
        ACL\_31 & 0.8406 & \textbf{0.8434} & 0.8325 & 0.8337 & 0.7976 \\
        ACL\_32$^{\dagger}$ & 0.8350 & 0.8352 & \textbf{0.8358} & 0.8339 & 0.7961 \\
        ACL\_34 & 0.8514 & \textbf{0.8515} & 0.8432 & 0.8460 & 0.7939 \\
        ACL\_2$^{\dagger}$ & 0.8031 & \textbf{0.8112} & 0.7918 & 0.8041 & 0.7909 \\
        ACL\_6$^{\dagger}$ & 0.8311 & \textbf{0.8316} & 0.8275 & 0.8109 & 0.7808 \\
        ACL\_13 & 0.8474 & \textbf{0.8477} & 0.8364 & 0.8433 & 0.7807 \\
        ACL\_17 & 0.8494 & 0.8483 & 0.8465 & \textbf{0.8495} & 0.7721 \\
        ACL\_3$^{\dagger}$ & 0.8213 & \textbf{0.8359} & 0.8302 & 0.8352 & 0.7624 \\
        ACL\_15 & \textbf{0.8550} & 0.8346 & 0.8490 & 0.8366 & 0.7624 \\
        ACL\_10 & \textbf{0.8489} & 0.8487 & 0.8474 & 0.8443 & 0.7611 \\
        ACL\_8 & \textbf{0.8568} & 0.8522 & 0.8517 & 0.8406 & 0.7578 \\
        ACL\_4$^{\dagger}$ & \textbf{0.8278} & 0.8067 & 0.7859 & 0.8081 & 0.7557 \\
        ACL\_19 & 0.8557 & \textbf{0.8571} & 0.8472 & 0.8530 & 0.7516 \\
        ACL\_28$^{\dagger}$ & \textbf{0.8217} & 0.8165 & 0.7820 & 0.8170 & 0.7475 \\
        ACL\_23$^{\dagger}$ & 0.8117 & \textbf{0.8150} & 0.8058 & 0.8029 & 0.7373 \\
        ACL\_12$^{\dagger}$ & \textbf{0.8320} & 0.8312 & 0.8270 & 0.8315 & 0.6897 \\
        ACL\_16$^{\dagger}$ & 0.8003 & \textbf{0.8140} & 0.7809 & 0.8105 & 0.5894 \\
        ACL\_35$^{\dagger}$ & \textbf{0.8183} & 0.8077 & 0.7855 & 0.8071 & 0.5487 \\
        \midrule
        \textbf{Average} & 0.8418 & 0.8412 & 0.8330 & 0.8368 & 0.7821 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Per-document COMET-Kiwi ↑ — ACL, Type 0 (sent) — sorted by ref}
    \label{tab:doc:acl:type_0:cometkiwi:sent}
    \medskip
    \raggedright\footnotesize
    Bold = best MT system per document.
    $^\dagger$ = document where the best MT score is worse than the global MT median.
\end{table}


==> tables/global_evaluation/global_evaluation_detail/ACL_cometkiwi_type_all.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrrr}
    \toprule
    \textbf{Document} & EuroLLM-22B-greedy & EuroLLM-9B-greedy & Llama-3.1-8B-greedy & Qwen3-8B-top-p & ref & ref\_sonnet \\
    \midrule
        ACL\_22 & \textbf{0.8643} & 0.8620 & 0.8503 & 0.8603 & 0.8573 & 0.8595 \\
        ACL\_18 & 0.8625 & \textbf{0.8642} & 0.8606 & 0.8582 & 0.8552 & 0.8588 \\
        ACL\_21 & \textbf{0.8558} & 0.8555 & 0.8487 & 0.8555 & 0.8479 & 0.8498 \\
        ACL\_25 & 0.8485 & \textbf{0.8559} & 0.8482 & 0.8500 & 0.8423 & 0.8488 \\
        ACL\_6 & \textbf{0.8442} & 0.8429 & 0.8335 & 0.8396 & 0.8353 & 0.8335 \\
        ACL\_1 & 0.8444 & \textbf{0.8493} & 0.8467 & 0.8434 & 0.8321 & 0.8289 \\
        ACL\_9 & \textbf{0.8369} & 0.8352 & 0.8322 & 0.8336 & 0.8308 & 0.8335 \\
        ACL\_5 & 0.8458 & \textbf{0.8460} & 0.8380 & 0.8404 & 0.8295 & 0.8373 \\
        ACL\_34 & 0.8432 & \textbf{0.8455} & 0.8313 & 0.8430 & 0.8280 & 0.8368 \\
        ACL\_17 & 0.8434 & \textbf{0.8449} & 0.8349 & 0.8397 & 0.8280 & 0.8323 \\
        ACL\_33 & 0.8447 & \textbf{0.8494} & 0.8398 & 0.8379 & 0.8269 & 0.8309 \\
        ACL\_12 & \textbf{0.8426} & 0.8422 & 0.8318 & 0.8371 & 0.8247 & 0.8309 \\
        ACL\_15 & \textbf{0.8446} & 0.8434 & 0.8367 & 0.8402 & 0.8233 & 0.8343 \\
        ACL\_0 & 0.8363 & \textbf{0.8390} & 0.8308 & 0.8319 & 0.8231 & 0.8231 \\
        ACL\_26 & 0.8401 & \textbf{0.8412} & 0.8300 & 0.8358 & 0.8224 & 0.8284 \\
        ACL\_27$^{\dagger}$ & \textbf{0.8321} & 0.8319 & 0.8109 & 0.8241 & 0.8200 & 0.8200 \\
        ACL\_14 & 0.8441 & \textbf{0.8451} & 0.8351 & 0.8411 & 0.8193 & 0.8322 \\
        ACL\_4 & \textbf{0.8417} & 0.8367 & 0.8271 & 0.8317 & 0.8183 & 0.8297 \\
        ACL\_24$^{\dagger}$ & 0.8303 & \textbf{0.8342} & 0.8251 & 0.8310 & 0.8182 & 0.8236 \\
        ACL\_30 & \textbf{0.8488} & 0.8438 & 0.8356 & 0.8426 & 0.8178 & 0.8300 \\
        ACL\_7 & \textbf{0.8384} & 0.8360 & 0.8277 & 0.8378 & 0.8176 & 0.8291 \\
        ACL\_8$^{\dagger}$ & 0.8290 & \textbf{0.8307} & 0.8154 & 0.8233 & 0.8172 & 0.8191 \\
        ACL\_11 & \textbf{0.8406} & 0.8402 & 0.8263 & 0.8341 & 0.8137 & 0.8274 \\
        ACL\_10$^{\dagger}$ & 0.8320 & \textbf{0.8339} & 0.8276 & 0.8296 & 0.8113 & 0.8216 \\
        ACL\_29$^{\dagger}$ & \textbf{0.8341} & 0.8322 & 0.8147 & 0.8270 & 0.8108 & 0.8164 \\
        ACL\_13 & 0.8365 & \textbf{0.8393} & 0.8287 & 0.8359 & 0.8099 & 0.8147 \\
        ACL\_32$^{\dagger}$ & \textbf{0.8341} & 0.8318 & 0.8264 & 0.8280 & 0.8087 & 0.8127 \\
        ACL\_23$^{\dagger}$ & 0.8322 & \textbf{0.8333} & 0.8206 & 0.8233 & 0.8071 & 0.8253 \\
        ACL\_19 & \textbf{0.8357} & 0.8333 & 0.8229 & 0.8321 & 0.8025 & 0.8120 \\
        ACL\_28$^{\dagger}$ & \textbf{0.8205} & 0.8205 & 0.8001 & 0.8203 & 0.8010 & 0.8116 \\
        ACL\_3 & 0.8295 & \textbf{0.8347} & 0.8257 & 0.8239 & 0.8002 & 0.8017 \\
        ACL\_20$^{\dagger}$ & 0.8157 & \textbf{0.8193} & 0.8046 & 0.8137 & 0.7997 & 0.8103 \\
        ACL\_31$^{\dagger}$ & 0.8155 & \textbf{0.8189} & 0.7996 & 0.8135 & 0.7961 & 0.8012 \\
        ACL\_2$^{\dagger}$ & 0.8031 & \textbf{0.8112} & 0.7918 & 0.8041 & 0.7909 & 0.7193 \\
        ACL\_35$^{\dagger}$ & \textbf{0.8150} & 0.8138 & 0.7962 & 0.8082 & 0.7814 & 0.7799 \\
        ACL\_16$^{\dagger}$ & 0.8018 & \textbf{0.8146} & 0.7973 & 0.8083 & 0.7639 & 0.7673 \\
        \midrule
        \textbf{Average} & 0.8363 & 0.8376 & 0.8265 & 0.8328 & 0.8176 & 0.8214 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Per-document COMET-Kiwi ↑ — ACL, All types (sent) — sorted by ref}
    \label{tab:doc:acl:all:cometkiwi:sent}
    \medskip
    \raggedright\footnotesize
    Bold = best MT system per document.
    $^\dagger$ = document where the best MT score is worse than the global MT median.
\end{table}

==> tables/global_evaluation/global_evaluation_detail/ACL_metricx_type_0.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Document} & EuroLLM-22B-greedy & EuroLLM-9B-greedy & Llama-3.1-8B-greedy & Qwen3-8B-top-p & ref \\
    \midrule
        ACL\_21 & 1.3576 & \textbf{1.3416} & 1.4092 & 1.4276 & 1.8147 \\
        ACL\_22 & \textbf{1.2913} & 1.3360 & 1.3972 & 1.4139 & 1.8835 \\
        ACL\_25 & 1.3086 & \textbf{1.1637} & 1.3698 & 1.2879 & 2.1099 \\
        ACL\_18 & 2.4188 & 2.3248 & 2.4357 & \textbf{2.3043} & 2.1861 \\
        ACL\_5 & 1.9629 & \textbf{1.7631} & 2.0055 & 1.8645 & 2.2451 \\
        ACL\_26 & 1.7191 & \textbf{1.6864} & 1.9099 & 1.8520 & 2.3982 \\
        ACL\_1 & 2.0459 & \textbf{1.8029} & 1.8900 & 1.9756 & 2.6882 \\
        ACL\_7 & 2.3190 & \textbf{2.1020} & 2.3898 & 2.2522 & 2.7973 \\
        ACL\_29 & 1.9505 & \textbf{1.9392} & 2.3291 & 2.3358 & 2.8570 \\
        ACL\_6 & 1.7479 & 1.6887 & \textbf{1.5547} & 2.0464 & 3.0072 \\
        ACL\_9$^{\dagger}$ & 2.8252 & \textbf{2.8190} & 2.9344 & 2.9406 & 3.0116 \\
        ACL\_10 & \textbf{1.5911} & 1.5940 & 1.6935 & 1.7857 & 3.0928 \\
        ACL\_0$^{\dagger}$ & \textbf{2.6510} & 2.7008 & 2.9426 & 2.8546 & 3.2197 \\
        ACL\_14 & 2.0025 & \textbf{1.8894} & 2.1846 & 1.9713 & 3.3130 \\
        ACL\_32$^{\dagger}$ & \textbf{2.4889} & 2.5705 & 2.6550 & 2.4951 & 3.3415 \\
        ACL\_8 & 1.6474 & \textbf{1.6406} & 1.6705 & 1.9065 & 3.3717 \\
        ACL\_30 & 1.8876 & \textbf{1.8525} & 1.8789 & 1.9555 & 3.4265 \\
        ACL\_24$^{\dagger}$ & \textbf{2.8535} & 2.9310 & 3.0511 & 2.9443 & 3.4607 \\
        ACL\_33$^{\dagger}$ & 2.7950 & \textbf{2.6142} & 2.9981 & 2.8316 & 3.5480 \\
        ACL\_15$^{\dagger}$ & \textbf{2.5837} & 2.5972 & 2.8040 & 2.6189 & 3.5505 \\
        ACL\_17$^{\dagger}$ & \textbf{2.5789} & 2.7952 & 2.7354 & 2.6114 & 3.6153 \\
        ACL\_13 & 2.1493 & \textbf{1.9519} & 2.3946 & 2.0769 & 3.6585 \\
        ACL\_11$^{\dagger}$ & 2.8996 & \textbf{2.8231} & 3.1013 & 2.8779 & 3.7967 \\
        ACL\_34 & 2.4388 & 2.4501 & 2.5829 & \textbf{2.4198} & 3.7991 \\
        ACL\_2$^{\dagger}$ & 3.4580 & \textbf{3.4421} & 3.7084 & 3.6853 & 3.9623 \\
        ACL\_31$^{\dagger}$ & 2.8316 & \textbf{2.6371} & 2.9133 & 2.8663 & 4.0176 \\
        ACL\_4 & \textbf{1.9847} & 2.1503 & 2.3778 & 2.0973 & 4.1464 \\
        ACL\_23$^{\dagger}$ & 2.8349 & \textbf{2.7020} & 3.1672 & 3.4020 & 4.4058 \\
        ACL\_12 & 2.3919 & \textbf{2.3544} & 2.5677 & 2.3854 & 4.4387 \\
        ACL\_3 & 2.4933 & \textbf{2.2429} & 2.7535 & 2.3822 & 4.5002 \\
        ACL\_20$^{\dagger}$ & \textbf{3.5054} & 3.8340 & 3.7285 & 3.9911 & 5.0611 \\
        ACL\_28$^{\dagger}$ & \textbf{3.1466} & 3.5056 & 3.9638 & 3.7157 & 5.1913 \\
        ACL\_19$^{\dagger}$ & \textbf{2.7545} & 2.8474 & 3.1629 & 3.0240 & 5.3003 \\
        ACL\_27 & 3.4414 & \textbf{2.2376} & 3.8945 & 2.9247 & 5.7746 \\
        ACL\_16 & \textbf{2.1407} & 2.2097 & 2.9265 & 2.4618 & 8.3304 \\
        ACL\_35$^{\dagger}$ & \textbf{3.4170} & 3.4290 & 4.0074 & 3.4743 & 10.5756 \\
        \midrule
        \textbf{Average} & 2.3865 & 2.3325 & 2.5969 & 2.4850 & 3.8305 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Per-document MetricX-QE ↓ — ACL, Type 0 (sent) — sorted by ref}
    \label{tab:doc:acl:type_0:metricxqe:sent}
    \medskip
    \raggedright\footnotesize
    Bold = best MT system per document.
    $^\dagger$ = document where the best MT score is worse than the global MT median.
\end{table}


==> tables/global_evaluation/global_evaluation_detail/ACL_metricx_type_all.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrrr}
    \toprule
    \textbf{Document} & EuroLLM-22B-greedy & EuroLLM-9B-greedy & Llama-3.1-8B-greedy & Qwen3-8B-top-p & ref & ref\_sonnet \\
    \midrule
        ACL\_25 & 1.7178 & \textbf{1.5396} & 1.6796 & 1.7032 & 1.8589 & 1.7622 \\
        ACL\_22 & \textbf{1.7488} & 1.8336 & 2.0594 & 1.9954 & 2.0147 & 1.9645 \\
        ACL\_18 & 2.0812 & \textbf{2.0272} & 2.1399 & 2.1107 & 2.0956 & 2.0455 \\
        ACL\_5 & 2.0568 & \textbf{2.0079} & 2.2108 & 2.0462 & 2.3025 & 2.1465 \\
        ACL\_26 & 2.1922 & \textbf{2.1347} & 2.3693 & 2.2578 & 2.4408 & 2.3532 \\
        ACL\_21 & 2.4118 & \textbf{2.1764} & 2.5609 & 2.4120 & 2.5015 & 2.3755 \\
        ACL\_6 & \textbf{2.2586} & 2.4675 & 2.6637 & 2.5566 & 2.5853 & 2.6846 \\
        ACL\_8 & \textbf{2.4341} & 2.4549 & 2.5436 & 2.6640 & 2.6697 & 2.8458 \\
        ACL\_1 & 2.0459 & \textbf{1.8029} & 1.8900 & 1.9756 & 2.6882 & 2.8107 \\
        ACL\_12 & 2.5387 & \textbf{2.4361} & 2.6878 & 2.6103 & 2.7547 & 2.7292 \\
        ACL\_9 & \textbf{2.6190} & 2.6766 & 2.7880 & 2.6608 & 2.7601 & 2.6662 \\
        ACL\_10 & 2.4142 & \textbf{2.2519} & 2.3116 & 2.3932 & 2.7893 & 2.5810 \\
        ACL\_7 & 2.4943 & \textbf{2.3724} & 2.7639 & 2.4465 & 2.8663 & 2.6251 \\
        ACL\_4 & 2.3782 & \textbf{2.3196} & 2.6429 & 2.5280 & 2.8730 & 2.6952 \\
        ACL\_27 & 2.5113 & \textbf{2.4817} & 3.0854 & 2.7811 & 2.8907 & 3.1373 \\
        ACL\_24$^{\dagger}$ & \textbf{2.7032} & 2.7466 & 2.9832 & 2.7603 & 2.9139 & 2.7733 \\
        ACL\_14 & 2.3574 & \textbf{2.2574} & 2.4712 & 2.4011 & 2.9291 & 2.6827 \\
        ACL\_15 & 2.6020 & 2.6118 & 2.7756 & \textbf{2.5988} & 2.9771 & 2.7685 \\
        ACL\_33 & 2.6717 & \textbf{2.5997} & 2.8689 & 2.7910 & 2.9917 & 2.9047 \\
        ACL\_11 & \textbf{2.2536} & 2.2556 & 2.6132 & 2.4220 & 3.0151 & 2.7004 \\
        ACL\_34$^{\dagger}$ & 2.7027 & \textbf{2.7000} & 2.9565 & 2.7553 & 3.0526 & 2.9019 \\
        ACL\_23$^{\dagger}$ & 2.8074 & \textbf{2.7615} & 3.2373 & 2.9456 & 3.1604 & 2.7532 \\
        ACL\_17$^{\dagger}$ & \textbf{3.0790} & 3.1429 & 3.5088 & 3.2317 & 3.2065 & 3.1263 \\
        ACL\_0 & \textbf{2.6510} & 2.7008 & 2.9426 & 2.8546 & 3.2197 & 3.2197 \\
        ACL\_32$^{\dagger}$ & \textbf{2.7305} & 2.8827 & 2.9962 & 2.8287 & 3.2525 & 3.2408 \\
        ACL\_30 & \textbf{2.5856} & 2.6586 & 2.8874 & 2.7623 & 3.2672 & 2.9836 \\
        ACL\_13$^{\dagger}$ & 2.7902 & 2.7918 & 2.9945 & \textbf{2.7867} & 3.3187 & 3.2282 \\
        ACL\_28$^{\dagger}$ & \textbf{3.0233} & 3.0423 & 3.2169 & 3.2622 & 3.5552 & 3.3327 \\
        ACL\_19$^{\dagger}$ & \textbf{2.8308} & 2.8826 & 3.0631 & 2.8710 & 3.5594 & 3.4729 \\
        ACL\_3 & 2.6731 & \textbf{2.6079} & 3.0861 & 3.0097 & 3.6737 & 3.6758 \\
        ACL\_29$^{\dagger}$ & \textbf{3.1960} & 3.2933 & 3.5384 & 3.4182 & 3.7572 & 3.5643 \\
        ACL\_31$^{\dagger}$ & 3.1782 & \textbf{3.0768} & 3.4616 & 3.2828 & 3.7923 & 3.6701 \\
        ACL\_2$^{\dagger}$ & 3.4580 & \textbf{3.4421} & 3.7084 & 3.6853 & 3.9623 & 5.4663 \\
        ACL\_35$^{\dagger}$ & \textbf{3.5079} & 3.5521 & 3.9235 & 3.6868 & 4.4308 & 4.4751 \\
        ACL\_16$^{\dagger}$ & \textbf{3.3446} & 3.4442 & 3.7089 & 3.6534 & 4.5497 & 4.5044 \\
        ACL\_20$^{\dagger}$ & \textbf{4.0124} & 4.0311 & 4.0375 & 4.2243 & 4.8794 & 4.8785 \\
        \midrule
        \textbf{Average} & 2.6406 & 2.6240 & 2.8716 & 2.7604 & 3.0988 & 3.0485 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Per-document MetricX-QE ↓ — ACL, All types (sent) — sorted by ref}
    \label{tab:doc:acl:all:metricxqe:sent}
    \medskip
    \raggedright\footnotesize
    Bold = best MT system per document.
    $^\dagger$ = document where the best MT score is worse than the global MT median.
\end{table}

==> tables/metric_results/main_results_moslem.tex <==




